A White Paper on Neural Network Quantization

While neural networks have advanced the frontiers in many applications, they often come at a high computational cost. Reducing the power and latency of neural network inference is key if we want to integrate modern networks into edge devices with strict power and compute requirements. Neural network quantization is one of the most effective ways of achieving these savings but the additional noise it induces can lead to accuracy degradation. In this white paper, we introduce state-of-the-art algorithms for mitigating the impact of quantization noise on the network's performance while maintaining low-bit weights and activations. We start with a hardware motivated introduction to quantization and then consider two main classes of algorithms: Post-Training Quantization (PTQ) and Quantization-Aware-Training (QAT). PTQ requires no re-training or labelled data and is thus a lightweight push-button approach to quantization. In most cases, PTQ is sufficient for achieving 8-bit quantization with close to floating-point accuracy. QAT requires fine-tuning and access to labeled training data but enables lower bit quantization with competitive results. For both solutions, we provide tested pipelines based on existing literature and extensive experimentation that lead to state-of-the-art performance for common deep learning models and tasks.

==> tables/03_AdaRound_extensions.tex <==
\begin{table}[t]
    \centering
    \caption{Top-1 ImageNet validation accuracy (in $\%$) for W4A8 post-training per-tensor quantization with base and extended variants of AdaRound.}
    \label{tbl:04_adaround_extensions}
    \begin{tabular}{ l c c c c }
         Method & ResNet-18 & ResNet-50 &  InceptionV3 & MobileNetV2 \\
         \midrule       
         Full Precision & 69.68 & 76.07 & 77.40 & 71.72 \\
         \midrule  
         Nearest (W4A32) & 23.99 & 35.60 & 1.67 & 8.09 \\
         AdaRound & 
            68.48$\pm{}$0.08 & 
            74.96$\pm{}$0.05 & 
            75.66$\pm{}$0.12 & 
            69.21$\pm{}$0.07 \\ 
         + extensions & 
            \textbf{68.74}$\pm{}$\textbf{0.07} & 
            \textbf{75.21}$\pm{}$\textbf{0.11} &
            \textbf{75.87}$\pm{}$\textbf{0.05} & 
            \textbf{69.54}$\pm{}$\textbf{0.11} \\ 
    \end{tabular}
\end{table}


\begin{table}%1
\tabcolsep8pt
%\noautomaticrules
\tabletitle{Comparison of MATLAB and C Code for Simple Matrix Operations}%
\begin{tabular}{@{}lccc@{}}
\tch{Operations}    &\tch{Part of C Code} &\tch{Hor. fts.} &\tch{Ver. fts.}\\[-2pt]
Ball &19, 221 &4, 598   &3, 200\\
Pepsi$^a$&46, 281 &6, 898 &5, 400\\
Keybrd$^b$   &27, 290 &2, 968 &3, 405\\
Pepsi    &14, 796 &9, 188 &3, 209\\
\end{tabular}
\end{table}

==> tables/03_CLE_ShuffleNetV2.tex <==
\begin{table}[t]
    \centering
    \caption{Top-1 ImageNet validation accuracy (in $\%$) for ShuffleNetV2, evaluated at full precision and 8-bit integer quantized}
     \label{tbl:04_cle_shufflenetv2}
    \begin{tabular}{ l r r }
         ShuffleNetV2          & \tt{x1.0}      & \tt{x0.5} \\
         \midrule       
         FP32 & 69.45 & 60.55 \\
         \midrule  
         Per-tensor quantization &  65.50 & 56.40 \\
         + DFQ   & 68.81   &  58.92  \\ 
         + CLE across blocks   & 68.92   &  \textbf{59.90}  \\ 
         \midrule
         Per-channel quantization & \textbf{69.00} & 59.87 \\
    \end{tabular}   
\end{table}


==> tables/03_adaround_intro.tex <==
\begin{table}[t]
    \centering
     \caption{Comparison of ImageNet validation accuracy between rounding-to-nearest vs 100 stochastic rounding choices. We report the mean and the standard deviation of 100 stochastic \cite{Gupta2015} rounding choices (Stochastic) as well as the best validation performance among these samples (Stochastic (best)).}
       \label{tab:adaround_introtable}
    \begin{tabular}{ l r }
         Rounding scheme          & Acc(\%)       \\\midrule
         Nearest            & 52.29  \\
         Stochastic         & 52.06$\pm$5.52   \\ 
         Stochastic (best)  & 63.06  \\
    \end{tabular}
\end{table}

==> tables/03_range_setting_activations.tex <==
\begin{table*}[t]
    \centering
     \tabletitle{Top-1 ImageNet validation accuracy (\%) for different methods of range setting of activation (symmetric uniform) quantizers while keeping the weights in FP32.}
     \label{tab:rangesetting_activations}
    \begin{tabular}{ l | r r r | r r r}
        Model (FP32 val accuracy) & \multicolumn{3}{c|}{\rn{18} (69.68\%)} & \multicolumn{3}{c}{\mnv{2} (71.72\%)} \\ \midrule
         Method/Bit-width           & 8    & 6      & 4    & 8 & 6    & 4 \\\midrule
         Min-Max         & 69.60$\pm$0.03         &       67.85$\pm$0.13   & 13.50$\pm$1.92   & 70.97$\pm$0.07         &  63.17$\pm$0.98  & 0.33$\pm$0.05\\
         MSE          & 69.44$\pm$0.10         & 64.09$\pm$1.05         & 15.06$\pm$1.55     & 71.15$\pm$0.16         &  63.85$\pm$1.60  & 8.08$\pm$0.13\\
         MSE + Xent         & 69.57$\pm$0.08         & 68.66$\pm$0.09         & 55.78$\pm$0.63     & 71.35$\pm$0.04         &  68.48$\pm$0.20  & 30.09$\pm$1.06\\
         BN ($\alpha=6$)& 69.63         & 68.17 & 18.29     & 71.2         &  64.82  & 0.50\\
    \end{tabular}
\end{table*} 
